Intelligent EHRs: Predicting Procedure Codes From Diagnosis Codes

In order to submit a claim to insurance companies, a doctor needs to code a patient encounter with both the diagnosis (ICDs) and procedures performed (CPTs) in an Electronic Health Record (EHR). Identifying and applying relevant procedures code is a cumbersome and time-consuming task as a doctor has to choose from around 13,000 procedure codes with no predefined one-to-one mapping. In this paper, we propose a state-of-the-art deep learning method for automatic and intelligent coding of procedures (CPTs) from the diagnosis codes (ICDs) entered by the doctor. Precisely, we cast the learning problem as a multi-label classification problem and use distributed representation to learn the input mapping of high-dimensional sparse ICDs codes. Our final model trained on 2.3 million claims is able to outperform existing rule-based probabilistic and association-rule mining based methods and has a recall of 90@3.

==> definitions.tex <==
%----------------------------------------------------------------
%  Definitions written by Sibt ul Hussain
\newif\ifwithlatentalgo
\newif\iflong
\newif\iflettrine
\newif\ifiksvm
\newif\ifaptable
\longtrue
\newif\ifmultitables
\multitablestrue
\newif\ifappendix
\appendixtrue
\newif\iflongtables
%--------------
\newif\ifltpap
\newif\ifnooverview
%---------------

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\usepackage{xspace}
\usepackage{upquote,textcomp}
\newcommand\upquote[1]{\textquotesingle#1\textquotesingle} % single quotes in better way ...

\def\bf#1{\textbf{#1}}
\def\ti#1{\textit{#1}}
\def\ie{\emph{i.e}\onedot}
\def\Ie{\emph{I.e}\onedot}

\def\wrt{\emph{w.r.t}\onedot}
\def\Wrt{\emph{W.r.t}\onedot}

\def\cf{\emph{c.f}\onedot}
\def\Cf{\emph{C.f}\onedot}

\def\etc{\emph{etc}\onedot}
\def\Etc{\emph{etc}\onedot}

\def\vs{\emph{vs}\onedot}

\def\Eg{\emph{E.g}\onedot}
\def\eg{\emph{e.g}\onedot}
\def\Eg{\emph{E.g}\onedot}

\def\etal{\emph{et al}\xspace}


\def\para#1{{\bf #1.}}
\def\mpara#1{\\\parskip{\bf #1.}\\\parindent}
%\long
\def\mbold#1{\textbf{#1}}
\def\mitalic#1{\textit{#1}}

\newif\ifwithcomments % by default false
\withcommentstrue
% \withcommentsfalse
\ifwithcomments

\long\def\comment#1{\para{\sffamily\{***\color{RoyalBlue}#1}****\} }% 
\long\def\question#1{\para{\textit\{???\color{Yellow}#1}????\} }
\long\def\discuss#1{{\color{ForestGreen}\mbold{\underline{DISCUSS:}}#1} }
\long\def\diagrams#1{\\{\color{Red}\mbold{\underline{Diagram:}}#1} }
\long\def\imp#1{{(\color{red}\mbold{\underline{#1}}} )}
\long\def\result#1{{\color{Red}#1}}
\long\def\idea#1{{\\\color{Magenta} \mbold{Idea:}#1}}
\long\def\revcomment#1{Reviewer BMVC:#1 }
\else

\long\def\comment#1{}
\long\def\discuss#1{ }
\long\def\revcomment#1{ }
\long\def\diagrams#1{ }
\long\def\idea#1{}
\fi
% LTP maps of data...
\def\pmap{\ensuremath{\overline{\Theta}_{r}^k}\xspace}
\def\nmap{\ensuremath{\underline{\Theta}_{r}^k}\xspace}
% color space definiations
\def\srgb{{sRGB}\xspace}
\def\rgb{{RGB}\xspace}
\def\xyz{{XYZ}\xspace}
\def\ocsa{{OCS}\xspace}
\def\ocs{{Opponent Color Space}\xspace}
\def\myverb#1{$#1$}
\def\l2norm{\mitalic{L2Norm}}
\def\stage#1{{Stage #1}\xspace}
%Feature names
\def\hog{HOG\xspace}
\def\hogx#1{$\text{\hog}_{#1}$}
\def\lbp{LBP\xspace}
\def\lbpltp{LBP+LTP\xspace}
\def\ltp{LTP\xspace}
\def\cslbp{CS-LBP\xspace}
\def\csltp{CS-LTP\xspace}
\def\lbphog{LBP+HOG\xspace}\def\ltphog{LTP+HOG\xspace} \def \lbpltphog{LBP+LTP+HOG\xspace}
\def\cslbphog{CS-LBP+HOG\xspace}\def\csltphog{CS-LTP+HOG\xspace} \def \cslbpltphog{CS-LBPLTP+HOG\xspace}
\def\cslbpltp{CS-LBPLTP\xspace}
% Referencing
\def\mcitep#1{\xspace\citep{#1}}
\def\C{{C}\xspace}
\def\J{{J}\xspace}
\newcommand{\mciteptw}[2]{~\citep{#1,#2}}
\newcommand{\mcitepth}[3]{~\citep{#1,#2,#3}}
\newcommand{\mcitepfo}[4]{~\citep{#1,#2,#3,#4}}
\newcommand{\mcitepfi}[5]{~\citep{#1,#2,#3,#4,#5}}


\newcommand{\mcite}[1]{\xspace\citet{#1}}
\newcommand{\mcitetw}[2]{~\citet{#1,#2}}
\newcommand{\mciteth}[3]{~\citet{#1,#2,#3}}
\newcommand{\mcitefo}[4]{~\citet{#1,#2,#3,#4}}
\newcommand{\mcitefi}[5]{~\citet{#1,#2,#3,#4,#5}}
% \newcommand{name}[num]{definition}
% \newcommand{name}[num]{definition}

% \def\mciteptw#2{~\citep{#1,#2}}
% \def\mcitepth#3{~\citep{#1,#2,#3}}
% \def\mcitepfo#4{~\citep{#1,#2,#3,#4}}
% \def\mcitepfi#5{~\citep{#1,#2,#3,#4,#5}}
% 
% 
%  \def\mcite#1{~\citet{#1}}
% \def\mcitetw#2{~\citet{#1,#2}}
% \def\mciteth#3{~\citet{#1,#2,#3}}
% \def\mcitefo#4{~\citet{#1,#2,#3,#4}}
% \def\mcitefi#5{~\citet{#1,#2,#3,#4,#5}}
\def\chref#1{Chapter~\ref{ch:#1}}
% \def\chrefcomb#2{Chapter~\ref{ch:#1} and ~\ref{ch:#2}}
\newcommand{\chrefcomb}[2]{Chapters~\ref{ch:#1} and ~\ref{ch:#2}}
\def\appref#1{Appendix~\ref{app:#1}}
\def\figref#1{Figure~\ref{figure:#1}}
% \def\figrefs#2{Figures~\ref{fig:#1} and \ref{fig:#2}}
\newcommand{\figrefs}[2]{Figures \ref{fig:#1} and \ref{fig:#2}}
\def\tabref#1{Table~\ref{table:#1}}
\def\secref#1{Sec.~\ref{sec:#1}}
\def\subsecref#1{SubSec.~\ref{subsec:#1}}
\def\eqref#1{Eq.~(\ref{eq:#1})}
\def\fppw{{FPPW}\xspace}
\def\fppws{{FPPWs}\xspace}
% tilde symbol
\def\ttilde{\ensuremath{\sim}}
\def\mtilde#1{\ensuremath{\tilde{#1}}}

% Accuracy Metrics
\def\apcomp {{Average Precision}\xspace}
\def\apcomps {{Average Precisions}\xspace}
\def\apcompsi {{Average Precisions}\xspace}
\def\ap{{AP}\xspace}
\def\aps{{APs}\xspace}
\def\map{{Mean AP}\xspace}
\def\det {{DET}\xspace}
\def\pr {{Precision{-}Recall}\xspace}
% Datasets
\def\inriads{INRIA\xspace}
\def\voc#1{VOC20#1\xspace}
\def\trnset{training set\xspace}
\def\tstset{test set\xspace}


%latentSVM
\def\latentsvm{{Latent SVM}\xspace}
% \def\rtemplate{\ensuremath{\rho}\xspace}
\def\fmap{$\varpi$\xspace}

\def\rtemplate{\ensuremath{{\boldsymbol{\rho}}}\xspace}
\def\fmap{\ensuremath{\boldsymbol{\varpi}}\xspace}
\def\windim{\ensuremath{w \times h}\xspace}

%Space in math mode
\def\ms{\:}
% Normalization definiations
\def\angle{ $\phi(i,j)$ }
\def\magnitude{ $\|\nabla(i,j)\|$ }
\def\rresult#1{\\{\color{Red}\mbold{\underline{Results???:}}#1} }

%normalizations
\newcommand{\ltwo}{\ensuremath{L_{2}}\xspace}
\newcommand{\lnorm}[1]{\ensuremath{L_{#1}}\xspace}
\newcommand{\lognorm}{Log\ensuremath{_{2}}\xspace}
\newcommand{\losqrt}[1]{\ensuremath{L_{#1}}-Sqrt\xspace}
\newcommand{\lpnorm}[1]{\ensuremath{\left\| #1 \right\|}\xspace}
\def\inriap{INRIA Person\xspace}
%compactlist
% Algorithm Details
\newenvironment{compactlistlone}
{\begin{compactenum}[(a)]}{\end{compactenum}}
\newenvironment{compactlistltwo}
{\begin{compactenum}[(1)]}{\end{compactenum}}
\newenvironment{compactlistlthree}
{\begin{compactenum}[(i)]}{\end{compactenum}}
\newenvironment{compactliststep}
{\begin{compactenum}[\hspace{0.2cm}Step 1.]}{\end{compactenum}}


% \def\in{\textbf{Input: }}
% \def\out{\textbf{Output: }}
\def\reducespace{\vspace{-12pt}}


% detectors
\def\winclass{{window-level classifier}\xspace}
\def\winc{{window-level}\xspace}
\def\winclasss{{window-level classifiers}\xspace}
\def\windet{{non-latent detector}\xspace}
\def\wind{{non-latent}\xspace}
\def\windets{{non-latent detectors}\xspace}
%\newcommand{\windet}[1]{window-classifier#1\xspace}
%\def\compdet{\mitalic{window-detector}\xspace}
\def\latentdet{{latent detector}\xspace}
\def\latentd{{latent}\xspace}
\def\latentdets{{latent detectors}\xspace}
\def\featpym{feature-pyramid\xspace}
\def\svm{SVM\xspace}
%space
\def\ospace#1{\ensuremath{\mathbb{R}^{#1}}\xspace}
\def\uspace#1{\ensuremath{\mathbb{R}_{#1}}\xspace}
% sparsification method...
\def\ism{IWT\xspace}
\def\nism{WT\xspace}
% seconds for the timing 
\def\sec{seconds\xspace}
% \def\min{\mitalic{min}\xspace}
% \def\cfbill{{\textbf{\sffamily\{***\textit{Check this line/section}}***\}}\xspace}
% \def\cfbillt#1{{\textbf{\sffamily\{***\textit{#1}}***\}}\xspace}

% \def\cfbill{\ensuremath{rightarrow}\xspace}
%matrices
\def\mat#1{\ensuremath{\mathbf #1}\xspace}
% A to Z
\def\mA{\ensuremath{\mat{A}}\xspace}
\def\mB{\ensuremath{\mat{B}}\xspace}
\def\mC{\ensuremath{\mat{C}}\xspace}
\def\mD{\ensuremath{\mat{D}}\xspace}
\def\mE{\ensuremath{\mat{E}}\xspace}
\def\mF{\ensuremath{\mat{F}}\xspace}
\def\mG{\ensuremath{\mat{G}}\xspace}
\def\mH{\ensuremath{\mat{H}}\xspace}
\def\mI{\ensuremath{\mat{I}}\xspace}
\def\mJ{\ensuremath{\mat{J}}\xspace}
\def\mK{\ensuremath{\mat{K}}\xspace}
\def\mL{\ensuremath{\mat{L}}\xspace}
\def\mM{\ensuremath{\mat{M}}\xspace}
\def\mN{\ensuremath{\mat{N}}\xspace}
\def\mO{\ensuremath{\mat{O}}\xspace}
\def\mP{\ensuremath{\mat{P}}\xspace}
\def\mQ{\ensuremath{\mat{Q}}\xspace}
\def\mR{\ensuremath{\mat{R}}\xspace}
\def\mS{\ensuremath{\mat{S}}\xspace}
\def\mT{\ensuremath{\mat{T}}\xspace}
\def\mU{\ensuremath{\mat{U}}\xspace}
\def\mV{\ensuremath{\mat{V}}\xspace}
\def\mW{\ensuremath{\mat{W}}\xspace}
\def\mX{\ensuremath{\mat{X}}\xspace}
\def\mY{\ensuremath{\mat{Y}}\xspace}
\def\mZ{\ensuremath{\mat{Z}}\xspace}

%Vectors
\def\vec#1{\ensuremath{\mathbf #1}\xspace}
% A to Z
\def\va{\ensuremath{\vec{a}}\xspace}
\def\vb{\ensuremath{\vec{b}}\xspace}
\def\vc{\ensuremath{\vec{c}}\xspace}
\def\vd{\ensuremath{\vec{d}}\xspace}
\def\ve{\ensuremath{\vec{e}}\xspace}
\def\vf{\ensuremath{\vec{f}}\xspace}
\def\vg{\ensuremath{\vec{g}}\xspace}
\def\vh{\ensuremath{\vec{h}}\xspace}
\def\vi{\ensuremath{\vec{i}}\xspace}
\def\vj{\ensuremath{\vec{j}}\xspace}
\def\vk{\ensuremath{\vec{k}}\xspace}
\def\vl{\ensuremath{\vec{l}}\xspace}
\def\vm{\ensuremath{\vec{m}}\xspace}
\def\vn{\ensuremath{\vec{n}}\xspace}
\def\vo{\ensuremath{\vec{o}}\xspace}
\def\vp{\ensuremath{\vec{p}}\xspace}
\def\vq{\ensuremath{\vec{q}}\xspace}
\def\vr{\ensuremath{\vec{r}}\xspace}
\def\vs{\ensuremath{\vec{s}}\xspace}
\def\vt{\ensuremath{\vec{t}}\xspace}
\def\vu{\ensuremath{\vec{u}}\xspace}
\def\vv{\ensuremath{\vec{v}}\xspace}
\def\vw{\ensuremath{\vec{w}}\xspace}
\def\vx{\ensuremath{\vec{x}}\xspace}
\def\vy{\ensuremath{\vec{y}}\xspace}
\def\vz{\ensuremath{\vec{z}}\xspace}

\def\vP{\ensuremath{\vec{P}}\xspace}
\newcommand{\tquote}[2]{
\begin{flushright}
\emph{#2}\newline
\hfill #1
\end{flushright}
\vspace{1cm}
}
\newcommand{\mquote}[1]{
\begin{center}
    \vspace{12pt}
\parbox{0.8\textwidth}{ #1 }
    \vspace{12pt}
\end{center}
}

%% Row counters example taken from latex matters http://texblog.wordpress.com/2007/07/25/counters-in-latex/
\newcounter{rno}
\newcommand{\newrow}[1]{
\refstepcounter{rno}\label{row:#1}\therno
}
\def\rowref#1{row~\ref{row:#1}}
\newcommand{\rowsref}[2]{
rows~\ref{row:#1} and~\ref{row:#2}}
\newcommand{\rowsrefwn}[2]{
\ref{row:#1} and~\ref{row:#2}
}
\def\kmeans{{K-Means}\xspace}
\def\lqp{LQP\xspace}
\def\lqphog{LQP+HOG\xspace}
\def\pls{PLS\xspace}
\def\fppi{{False Positive Per Image}\xspace}
% \def\ff{\ensuremath{_{ff}}}
% \def\mf{\ensuremath{_{mf}}}
\def\ff{\ensuremath{_{f}}}
\def\mr#1{#1Root\xspace}
\def\lf{{left facing}\xspace}
\def\rf{{right facing}\xspace}
\def\ffr#1{#1Root\ff\xspace}
\def\ffrp#1{#1Root\ff\ensuremath{\times6}Part\xspace}
\def\rfppi{Recall-\fppi}
\def\srp{6Root\ensuremath{\times8}Part\xspace}
\def\fwt{FWT\xspace}
\def\lo{$L_1$\xspace}
\def\lt{$L_2$\xspace}
\def\imgext{.png}

\def\fft{{folding}\xspace}
\def\mft{{mirroring}\xspace}
\def\mrff{{MR-flipfold}\xspace}
\def\mrmf{{MR-mirrorflip}\xspace}

\def\B#1{\textbf{#1}}
\def\tss#1{\textsuperscript{#1}}

\def\mytstrut{\vphantom{$()^{()}$}}
\def\mybstrut{\vphantom{$()_{()}$}}
\def\mystrut{\vphantom{$X_{()}^{()}$}}
\def\ti#1{\emph{#1}}

\newcommand{\qf}[3]{#1\ensuremath{_{#2}^{#3}}\xspace}
\def\kmeans{K-means\xspace}
\newcommand{\uline}[1]{\rule[0pt]{#1}{0.4pt}}% Fill this blank
%fill with lines 
\newcommand{\lines}[1]{
 \setlength\linefillheight{.3in}
\fillwithlines{#1in}}
\definecolor{bg}{rgb}{0.95,0.95,0.95} % background colour used for minted environments...



% Minted commands for syntax highlighting -- see the minted.sty manual for further information
% 
% \newminted{cpp}{linenos,
%                numbersep=8pt,
%                frame=lines,
%                framesep=2mm,
%                bgcolor=bg}
% \newminted{bash}{linenos,
%                numbersep=8pt,
%                frame=lines,
%                framesep=2mm,
%                bgcolor=bg}
% \newmint{bash}{linenos,
%                numbersep=8pt,
%                frame=lines,
%                framesep=2mm,
%                bgcolor=bg}
% \newmint{cpp}{linenos,
%                numbersep=8pt,
%                frame=lines,
%                framesep=2mm,
%                bgcolor=bg}  
